Averaging Attacks on Bounded Noise-based Disclosure Control Algorithms

We describe and evaluate an attack that reconstructs the histogram of any target attribute of a sensitive dataset which can only be queried through a specific class of real-world privacy-preserving algorithms which we call bounded perturbation algorithms. A defining property of such an algorithm is that it perturbs answers to the queries by adding zero-mean noise distributed within a bounded (possibly undisclosed) range. Other key properties of the algorithm include only allowing restricted queries (enforced via an online interface), suppressing answers to queries which are only satisfied by a small group of individuals (e.g., by returning a zero as an answer), and adding the same perturbation to two queries which are satisfied by the same set of individuals (to thwart differencing or averaging attacks). A real-world example of such an algorithm is the one deployed by the Australian Bureau of Statistics' (ABS) online tool called TableBuilder, which allows users to create tables, graphs and maps of Australian census data [30]. We assume an attacker (say, a curious analyst) who is given oracle access to the algorithm via an interface. We describe two attacks on the algorithm. Both attacks are based on carefully constructing (different) queries that evaluate to the same answer. The first attack finds the hidden perturbation parameter $r$ (if it is assumed not to be public knowledge). The second attack removes the noise to obtain the original answer of some (counting) query of choice. We also show how to use this attack to find the number of individuals in the dataset with a target attribute value $a$ of any attribute $A$, and then for all attribute values $a_i \in A$. Our attacks are a practical illustration of the (informal) fundamental law of information recovery which states that ``overly accurate estimates of too many statistics completely destroys privacy'' [9, 15].

==> results-table.tex <==
%!TEX root = nonoise.tex

%\begin{tabularx}{\textwidth}{ l | l | l | l | l | l | l }
\begin{longtable}{ p{.1\textwidth} | p{.1\textwidth} | p{.1\textwidth} | p{.1\textwidth} | p{.1\textwidth} | p{.1\textwidth} | p{.1\textwidth}} 
\caption{Results of running Attack 2 to retrieve a target column of the synthetic dataset. }
\label{tab:results}
\endfirsthead
\endhead
	Att. value & Actual & Noisy & $t = 50$ & $t = 127$ & $t = 200$ & $t = 255$ \\ 
	\hline\hline
	1 & 1 & suppressed & 1 & 1 & 1 & 1 \\ \hline
	2 & 3 & 0 & 3 & 3 & 3 & 3 \\ \hline
	3 & 6 & 6 & 6 & 6 & 6 & 6 \\ \hline
	4 & 12 & 12 & 12 & 12 & 12 & 12 \\ \hline
	5 & 33 & 34 & 33 & 33 & 33 & 33 \\ \hline
	6 & 114 & 116 & 114 & 114 & 114 & 114 \\ \hline
	7 & 199 & 197 & 199 & 199 & 199 & 199 \\ \hline
	8 & 372 & 373 & 372 & 372 & 372 & 372 \\ \hline
	9 & 677 & 678 & \textcolor{red}{678} & 677 & 677 & 677 \\ \hline
	10 & 1075 & 1074 & 1075 & 1075 & 1075 & 1075 \\ \hline
	11 & 2884 & 2883 & 2884 & 2884 & 2884 & 2884 \\ \hline
	12 & 4388 & 4389 & 4388 & 4388 & 4388 & 4388 \\ \hline
	13 & 6496 & 6495 & 6496 & 6496 & 6496 & 6496 \\ \hline
	14 & 9136 & 9137 & 9136 & 9136 & 9136 & 9136 \\ \hline
	15 & 12694 & 12692 & \textcolor{red}{12693} & 12694 & 12694 & 12694 \\ \hline
	16 & 16893 & 16892 & 16893 & 16893 & 16893 & 16893 \\ \hline
	17 & 21513 & 21515 & 21513 & 21513 & 21513 & 21513 \\ \hline
	18 & 26566 & 26564 & 26566 & 26566 & 26566 & 26566 \\ \hline
	19 & 31854 & 31853 & 31854 & 31854 & 31854 & 31854 \\ \hline
	20 & 36741 & 36739 & 36741 & 36741 & 36741 & 36741 \\ \hline
	21 & 40268 & 40267 & 40268 & 40268 & 40268 & 40268 \\ \hline
	22 & 43426 & 43427 & 43426 & 43426 & 43426 & 43426 \\ \hline
	23 & 44865 & 44867 & 44865 & 44865 & 44865 & 44865 \\ \hline
	24 & 44812 & 44813 & 44812 & 44812 & 44812 & 44812 \\ \hline
	25 & 43054 & 43053 & 43054 & 43054 & 43054 & 43054 \\ \hline
	26 & 35698 & 35696 & 35698 & 35698 & 35698 & 35698 \\ \hline
	27 & 31534 & 31532 & \textcolor{red}{31535} & 31534 & 31534 & 31534 \\ \hline
	28 & 26103 & 26105 & 26103 & 26103 & 26103 & 26103 \\ \hline
	29 & 20953 & 20955 & 20953 & 20953 & 20953 & 20953 \\ \hline
	30 & 12430 & 12431 & 12430 & 12430 & 12430 & 12430 \\ \hline
	31 & 8977 & 8975 & 8977 & 8977 & 8977 & 8977 \\ \hline
	32 & 6297 & 6296 & 6297 & 6297 & 6297 & 6297 \\ \hline
	33 & 2715 & 2713 & 2715 & 2715 & 2715 & 2715 \\ \hline
	34 & 1775 & 1774 & 1775 & 1775 & 1775 & 1775 \\ \hline
	35 & 1085 & 1084 & 1085 & 1085 & 1085 & 1085 \\ \hline
	36 & 614 & 615 & 614 & 614 & 614 & 614 \\ \hline
	37 & 377 & 378 & 377 & 377 & 377 & 377 \\ \hline
	38 & 196 & 195 & 196 & 196 & 196 & 196 \\ \hline
	39 & 53 & 52 & 53 & 53 & 53 & 53 \\ \hline
	40 & 24 & 25 & 24 & 24 & 24 & 24 \\ \hline
	41 & 14 & 15 & 14 & \textcolor{red}{13} & 14 & 14 \\ \hline
	42 & 3 & 0 & 3 & 3 & 3 & 3 \\ \hline
	43 & 4 & 0 & 4 & 4 & 4 & 4 \\ \hline
	44 & 1 & suppressed & 1 & 1 & 1 & 1 \\ \hline
	45 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	46 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	47 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	48 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	49 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	50 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	51 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	52 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	53 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	54 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	55 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	56 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	57 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	58 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	59 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	60 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	62 & 0 & 0 & \textcolor{red}{-1} & 0 & 0 & 0 \\ \hline
	63 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	64 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	66 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	67 & 0 & 0 & \textcolor{red}{-1} & 0 & 0 & 0 \\ \hline
	69 & 0 & 0 & \textcolor{red}{-1} & 0 & 0 & 0 \\ \hline
	70 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	72 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	73 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	75 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	76 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	77 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	80 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	81 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	82 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	84 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	85 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	86 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	87 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	89 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	90 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	91 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	92 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	94 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	95 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	96 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	99 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	A0 & 0 & 0 & 0 & \textcolor{red}{-1} & 0 & 0 \\ \hline
	B0 & 53 & 52 & 53 & 53 & 53 & 53 \\ \hline
	C0 & 1837 & 1838 & 1837 & 1837 & 1837 & 1837 \\ \hline
	D0 & 40259 & 40258 & 40259 & 40259 & 40259 & 40259 \\ \hline
	E0 & 16539 & 16537 & 16539 & 16539 & 16539 & 16539 \\ \hline
	F0 & 4283 & 4284 & 4283 & 4283 & 4283 & 4283 \\ \hline
	G0 & 93 & 95 & 93 & 93 & 93 & 93 \\ \hline
	H0 & 1 & suppressed & 1 & 1 & 1 & 1 \\ \hline
	I0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	J0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	K0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	L0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	M0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	N0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	O0 & 0 & 0 & \textcolor{red}{1} & 0 & 0 & 0 \\ \hline
	P0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	Q0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	R0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	S0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
	VV & 0 & 0 & \textcolor{red}{-1} & 0 & 0 & 0 \\ \hline\hline
Error rate & - & - & 7.48\% & 1.87\% & 0\% & 0\% 
\end{longtable}
